Formally Specifying and Proving Operational Aspects of Forensic Lucid in Isabelle

A Forensic Lucid intensional programming language has been proposed for intensional cyberforensic analysis. In large part, the language is based on various predecessor and codecessor Lucid dialects bound by the higher-order intensional logic (HOIL) that is behind them. This work formally specifies the operational aspects of the Forensic Lucid language and compiles a theory of its constructs using Isabelle, a proof assistant system.

==> Makefile <==
# $Header: /cvsroot/publications/2008/flucid-isabelle-tphols08/Makefile,v 1.2 2008/01/28 22:25:07 mokhov Exp $

#
# Settings
#

#PDFLATEXFLAGS = --interaction=batchmode --file-line-error-style
PDFLATEXFLAGS = --interaction=batchmode

DELIVERABLE = flucid-isabelle-tphols08
SUBMISSIONDIR = flucid-isabelle-tphols08-public

IPLEXAMPLEFILES := multilang language-mix

JAVAEXAMPLEFILES :=
TEXTEXAMPLEFILES :=

IPLFILES := $(IPLEXAMPLEFILES:%=%.ipl)
JAVAFILES := $(JAVAEXAMPLEFILES:%=%.java)
TEXTFILES := $(TEXTEXAMPLEFILES:%=%.txt)

TEXJAVAFILES := $(JAVAEXAMPLEFILES:%=%.tex)
TEXIPLFILES := $(IPLEXAMPLEFILES:%=%.tex)
TEXTEXTFILES := $(TEXTEXAMPLEFILES:%=%.tex)

#
# Build
#

all: $(DELIVERABLE).pdf

$(DELIVERABLE).pdf: $(DELIVERABLE).tex $(DELIVERABLE).bib commands.tex #date.tex examples
	@echo "Compiling *.tex files..."
	pdflatex $(PDFLATEXFLAGS) $(DELIVERABLE)
	@echo "Compiling bibliography..."
	bibtex $(DELIVERABLE)
	@echo "Updating cross-references..."
	pdflatex $(PDFLATEXFLAGS) $(DELIVERABLE)
	pdflatex $(PDFLATEXFLAGS) $(DELIVERABLE)

$(DELIVERABLE).bib:
# $(DELIVERABLE).bib: ../../../common/bibliography.bib
# 	ln -sf ../../../common/bibliography.bib $(DELIVERABLE).bib

date.tex:
	@echo "Time-stamping..."
	date > date.tex

submission: all
	mkdir -p $(SUBMISSIONDIR)
	cp Makefile *.tex *.bib *.pdf *.png *.ipl *.java $(SUBMISSIONDIR)
	make -C $(SUBMISSIONDIR) clean
	tar cvf $(SUBMISSIONDIR).tar $(SUBMISSIONDIR)
	gzip --best $(SUBMISSIONDIR).tar

examples: $(TEXIPLFILES) $(TEXJAVAFILES)

$(TEXJAVAFILES): $(JAVAFILES)
	@echo "Doing $@..."
	@echo "\begin{verbatim}" > $@
	@cat `echo $@ | sed -e "s/tex/java/"` | perl -e "while(<STDIN>){s/\t/    /g; print}" >> $@
	@echo "\end{verbatim}" >> $@

$(TEXIPLFILES): $(IPLFILES)
	@echo "Doing $@..."
	@echo "\begin{verbatim}" > $@
	@cat `echo $@ | sed -e "s/tex/ipl/"` | grep -v 'Header' | grep -v 'Id' | grep -v 'Date' | grep -v 'Revision' | perl -e "while(<STDIN>){s/\t/    /g; print}" >> $@
	@echo "\end{verbatim}" >> $@

$(TEXTEXTFILES): $(TEXTFILES)
	@echo "Doing $@..."
	@echo "\begin{verbatim}" > $@
	@cat `echo $@ | sed -e "s/tex/txt/"` | perl -e "while(<STDIN>){s/\t/    /g; print}" >> $@
	@echo "\end{verbatim}" >> $@

#
# Clean up
#

clean:
	rm -f *~ *.log *.dvi *.aux date.tex *.toc \
          *.lot *.lof *.idx *.bbl *.blg *.ilg *.ind \
          genST-short.tex genST-long.tex \
          genST-short.java genST-long.java \
          $(TEXIPLFILES) \
          $(TEXJAVAFILES) \
          $(TEXTEXTFILES)

maintainer-clean: clean
	rm -f *.pdf

# EOF

